Adaptive Beam Tracking based on Recurrent Neural Networks for mmWave Channels

The performance of millimeter wave (mmWave) communications critically depends on the accuracy of beamforming both at base station (BS) and user terminals (UEs) due to high isotropic path-loss and channel attenuation. In high mobility environments, accurate beam alignment becomes even more challenging as the angles of the BS and each UE must be tracked reliably and continuously. In this work, focusing on the beamforming at the BS, we propose an adaptive method based on Recurrent Neural Networks (RNN) that tracks and predicts the Angle of Departure (AoD) of a given UE. Moreover, we propose a modified frame structure to reduce beam alignment overhead and hence increase the communication rate. Our numerical experiments in a highly non-linear mobility scenario show that our proposed method is able to track the AoD accurately and achieve higher communication rate compared to more traditional methods such as the particle filter.

==> Neuer Ordner/FrameTimeSlots.tex <==
%\begin{tikzpicture}
%    [%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%        box/.style={rectangle,draw=black, ultra thick, minimum size=1cm},
%    ]%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    
%    
%    
%\tikzset{
%  boxy/.style = {rectangle,
%    draw=black,
%     ultra thick, 
%     minimum size=1cm ,
%     fill=blue!30
%  }
%}
%
%\newcommand{\mywind}[1]{\node [mywind] }
%    
%%    
%%      \newcommand*{\mywind}[1]{ [
%%        box/.style={rectangle,draw=red, ultra thick, minimum size=1cm},]}
%%    
%%     \newcommand*{\mywinds}[1]{\fcolorbox{red}{red!20!white}{$#1$}}
%
%\foreach \x/\y in {0/0, 3/,6/ ,9/G-1}
%        \node[box] at (\x,0){\y};
%        
%%        \foreach \x/\y in {3/k-L,4/,5/k,6/,7/k+L}
%%        \node[boxy] at (\x,0){\y};
%        
%        \foreach \x/\y in {3/0,4/0,5/0,6/1,7/0}
%        \node[box] at (\x,-3){\y};
%      
%
%
%%\draw[decorate,decoration={brace,mirror},thick] (2.5,-.7) -- node[below]{sliding feature window (input features)} (7.5,-.7);
%%\draw[decorate,decoration={brace,mirror},thick] (-.5,-1.5) -- node[below]{pseudo-spectrum} (10.5,-1.50);
%%\draw[->,very thick] (3,1.2) --  node[above,yshift=2mm]{last element in window} (3,.7);
%%\draw[->,very thick] (5,1.4) --  node[above,yshift=4.5mm]{CUT} (5,.7);
%%
%%\draw[<-, thick] (8,-3.0) --  node[right,xshift=3mm, yshift=0mm]{label vector} (8.5,-3.0);
%%\draw[<-, thick] (8,-3) --  node[right,yshift=1mm]{input features} (8.5,-3);
%
%\end{tikzpicture}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usetikzlibrary{arrows.meta,shapes.arrows,chains,decorations.pathreplacing}

\newlength\myht
\settoheight{\myht}{$n-2$}
\tikzset{%
  MyStyle/.style={draw, text width=80pt, text height=10pt, text centered,minimum height=\myht+2*3*1mm)},
  MyStylef/.style={draw, text width=60pt, text height=10pt, text centered,minimum height=\myht+2*3*1mm)},
  MyStyleD/.style={draw, text width=180pt, text height=10pt, text centered,minimum height=\myht+3*2*1mm)},
  MyStyleE/.style={draw, text width=15pt, text height=10pt, text centered,minimum height=\myht+2*3*1mm)},
  MyStyleS/.style={draw, text width=40pt, text height=10pt, text centered,minimum height=\myht+2*3*1mm)},
  boxy/.style = {rectangle,draw=black, minimum height=\myht+2*3*1mm ,fill=blue!20},
  boxy2/.style = {rectangle,draw=black, minimum height=\myht+2*3*1mm ,fill=red!20},
  myarrow/.style={shape=single arrow, rotate=90, inner sep=5pt, outer sep=0pt, single arrow head extend=0pt, minimum height=7.5pt, text width=0pt, draw=blue!50, fill=blue!25}
}

\begin{tikzpicture}[-{Stealth[length=2.5pt]}]
  \begin{scope} [shift={(-2,0)},name=scope1,start chain, node distance=-.5pt]
    \foreach \name [count=\xi] in {1}{ \node[MyStyle, on chain] (vlos\xi) {Initial BA};}
     \foreach \name [count=\xi] in {1}{ \node[MyStylef, on chain] (vlosf\xi) {UL-FB};}
     \foreach \name [count=\xi] in {1}{ \node[MyStyleD, on chain] (vlosD\xi) {Data Transmission (DL)};}
     \foreach \name [count=\xi] in {1}{ \node[boxy, on chain] (vlosE\xi) {SP};}
  \end{scope}
  \node[above= 0.1cm of vlos1, xshift=-0.2cm]{$T_{ACQ}$};
   \node[above= 0.1cm of vlosf1, xshift=-0.0cm]{$T_{FB,I}$};
    \node[above= 0.1cm of vlosD1, xshift=-0.5cm]{$T_{DL}$};
    \node[above= 0.1cm of vlosE1, xshift=0.0cm]{$T_{SP}$};

  \draw [decorate,decoration={brace,amplitude=10pt,mirror}]
  (vlos1.south west) -- (vlosE1.south east) node[black,midway,below=7pt]
  {T$_F$};
%\end{tikzpicture}
%

%\begin{tikzpicture}[-{Stealth[length=2.5pt]}]
  \begin{scope} [shift={(-2.85,-2.5)}, start chain, node distance=-.5pt]
    \foreach \name [count=\xi] in {2}{ \node[boxy, on chain] (vlosf\xi) {UL-FB};}
     \foreach \name [count=\xi] in {2}{ \node[MyStyleD, on chain] (vlosD\xi) {Data Transmission (DL)};}
     \foreach \name [count=\xi] in {2}{ \node[MyStyleE, on chain] (vlosE\xi) {SP};}
  \end{scope}
    \node[above= 0.1cm of vlosf1, xshift=-0.0cm]{$T_{FB,SP}$};
    \node[above= 0.1cm of vlosD1, xshift=-0.5cm]{$T_{DL}$};
    \node[above= 0.1cm of vlosE1, xshift=0.0cm]{$T_{SP}$};
    
      \draw [decorate,decoration={brace,amplitude=10pt,mirror}]
  (vlosf1.south west) -- (vlosE1.south east) node[black,midway,below=7pt]
  {T$_{F'}$};
  
  \node[draw] at (-5, 0)   (a) {(a)};
  \node[draw] at (-5, -2.5)   (b) {(b)};
%  \draw [decorate,decoration={brace,amplitude=10pt,mirror}]
%  (vlos7.south west) -- (vlos11.south east) node[black,midway,below=8pt]
%  {Removed data};
\end{tikzpicture}

%\begin{tikzpicture}[
%  -{Stealth[length=2.5pt]}
%  ]
%  \begin{scope} [start chain, node distance=-.5pt]
%    \foreach \name [count=\xi] in {1,2,3,\cdots,k,\cdots,n-k, \cdots,
%      n-2,n-1,n}{ \node[MyStyle, on chain] (vlos\xi) {$\name$};
%    }
%  \end{scope}
%  \node[above= 0.1cm of vlos1, xshift=-0.5cm]{$u_{bef}$};
%
%  \draw [decorate,decoration={brace,amplitude=10pt,mirror}]
%  (vlos1.south west) -- (vlos5.south east) node[black,midway,below=8pt]
%  {Removed data};
%\end{tikzpicture}































==> Neuer Ordner/macros.tex <==

%
\setlength\unitlength{1mm}

\newcommand{\insertfig}[3]{
\begin{figure}[htbp]\begin{center}\begin{picture}(120,90)
\put(0,-5){\includegraphics[width=12cm,height=9cm,clip=]{#1.eps}}\end{picture}\end{center}
\caption{#2}\label{#3}\end{figure}}

\newcommand{\insertxfig}[4]{
\begin{figure}[htbp]
\begin{center}
\leavevmode \centerline{\resizebox{#4\textwidth}{!}{\input
#1.pstex_t}}
%\vspace*{-0.2in}
\caption{#2} \label{#3}
\end{center}
\end{figure}}

\long\def\comment#1{}

% bb font symbols

\newfont{\bbb}{msbm10 scaled 700}
\newcommand{\CCC}{\mbox{\bbb C}}

\newfont{\bb}{msbm10 scaled 1100}
\newcommand{\CC}{\mbox{\bb C}}
\newcommand{\PP}{\mbox{\bb P}}
\newcommand{\RR}{\mbox{\bb R}}
\newcommand{\QQ}{\mbox{\bb Q}}
\newcommand{\ZZ}{\mbox{\bb Z}}
\newcommand{\FF}{\mbox{\bb F}}
\newcommand{\GG}{\mbox{\bb G}}
\newcommand{\EE}{\mbox{\bb E}}
\newcommand{\NN}{\mbox{\bb N}}
\newcommand{\KK}{\mbox{\bb K}}

% Vectors

\newcommand{\av}{{\bf a}}
\newcommand{\bv}{{\bf b}}
\newcommand{\cv}{{\bf c}}
\newcommand{\dv}{{\bf d}}
\newcommand{\ev}{{\bf e}}
\newcommand{\fv}{{\bf f}}
\newcommand{\gv}{{\bf g}}
\newcommand{\hv}{{\bf h}}
\newcommand{\iv}{{\bf i}}
\newcommand{\jv}{{\bf j}}
\newcommand{\kv}{{\bf k}}
\newcommand{\lv}{{\bf l}}
\newcommand{\mv}{{\bf m}}
\newcommand{\nv}{{\bf n}}
\newcommand{\ov}{{\bf o}}
\newcommand{\pv}{{\bf p}}
\newcommand{\qv}{{\bf q}}
\newcommand{\rv}{{\bf r}}
\newcommand{\sv}{{\bf s}}
\newcommand{\tv}{{\bf t}}
\newcommand{\uv}{{\bf u}}
\newcommand{\wv}{{\bf w}}
\newcommand{\vv}{{\bf v}}
\newcommand{\xv}{{\bf x}}
\newcommand{\yv}{{\bf y}}
\newcommand{\zv}{{\bf z}}
\newcommand{\zerov}{{\bf 0}}
\newcommand{\onev}{{\bf 1}}

% Matrices

\newcommand{\Am}{{\bf A}}
\newcommand{\Bm}{{\bf B}}
\newcommand{\Cm}{{\bf C}}
\newcommand{\Dm}{{\bf D}}
\newcommand{\Em}{{\bf E}}
\newcommand{\Fm}{{\bf F}}
\newcommand{\Gm}{{\bf G}}
\newcommand{\Hm}{{\bf H}}
\newcommand{\Id}{{\bf I}}
\newcommand{\Jm}{{\bf J}}
\newcommand{\Km}{{\bf K}}
\newcommand{\Lm}{{\bf L}}
\newcommand{\Mm}{{\bf M}}
\newcommand{\Nm}{{\bf N}}
\newcommand{\Om}{{\bf O}}
\newcommand{\Pm}{{\bf P}}
\newcommand{\Qm}{{\bf Q}}
\newcommand{\Rm}{{\bf R}}
\newcommand{\Sm}{{\bf S}}
\newcommand{\Tm}{{\bf T}}
\newcommand{\Um}{{\bf U}}
\newcommand{\Wm}{{\bf W}}
\newcommand{\Vm}{{\bf V}}
\newcommand{\Xm}{{\bf X}}
\newcommand{\Ym}{{\bf Y}}
\newcommand{\Zm}{{\bf Z}}

% Calligraphic

\newcommand{\Ac}{{\cal A}}
\newcommand{\Bc}{{\cal B}}
\newcommand{\Cc}{{\cal C}}
\newcommand{\Dc}{{\cal D}}
\newcommand{\Ec}{{\cal E}}
\newcommand{\Fc}{{\cal F}}
\newcommand{\Gc}{{\cal G}}
\newcommand{\Hc}{{\cal H}}
\newcommand{\Ic}{{\cal I}}
\newcommand{\Jc}{{\cal J}}
\newcommand{\Kc}{{\cal K}}
\newcommand{\Lc}{{\cal L}}
\newcommand{\Mc}{{\cal M}}
\newcommand{\Nc}{{\cal N}}
\newcommand{\Oc}{{\cal O}}
\newcommand{\Pc}{{\cal P}}
\newcommand{\Qc}{{\cal Q}}
\newcommand{\Rc}{{\cal R}}
\newcommand{\Sc}{{\cal S}}
\newcommand{\Tc}{{\cal T}}
\newcommand{\Uc}{{\cal U}}
\newcommand{\Wc}{{\cal W}}
\newcommand{\Vc}{{\cal V}}
\newcommand{\Xc}{{\cal X}}
\newcommand{\Yc}{{\cal Y}}
\newcommand{\Zc}{{\cal Z}}

% Bold greek letters

\newcommand{\alphav}{\hbox{\boldmath$\alpha$}}
\newcommand{\betav}{\hbox{\boldmath$\beta$}}
\newcommand{\gammav}{\hbox{\boldmath$\gamma$}}
\newcommand{\deltav}{\hbox{\boldmath$\delta$}}
\newcommand{\etav}{\hbox{\boldmath$\eta$}}
\newcommand{\lambdav}{\hbox{\boldmath$\lambda$}}
\newcommand{\epsilonv}{\hbox{\boldmath$\epsilon$}}
\newcommand{\nuv}{\hbox{\boldmath$\nu$}}
\newcommand{\muv}{\hbox{\boldmath$\mu$}}
\newcommand{\zetav}{\hbox{\boldmath$\zeta$}}
\newcommand{\phiv}{\hbox{\boldmath$\phi$}}
\newcommand{\psiv}{\hbox{\boldmath$\psi$}}
\newcommand{\thetav}{\hbox{\boldmath$\theta$}}
\newcommand{\tauv}{\hbox{\boldmath$\tau$}}
\newcommand{\omegav}{\hbox{\boldmath$\omega$}}
\newcommand{\xiv}{\hbox{\boldmath$\xi$}}
\newcommand{\sigmav}{\hbox{\boldmath$\sigma$}}
\newcommand{\piv}{\hbox{\boldmath$\pi$}}
\newcommand{\rhov}{\hbox{\boldmath$\rho$}}

\newcommand{\Gammam}{\hbox{\boldmath$\Gamma$}}
\newcommand{\Lambdam}{\hbox{\boldmath$\Lambda$}}
\newcommand{\Deltam}{\hbox{\boldmath$\Delta$}}
\newcommand{\Sigmam}{\hbox{\boldmath$\Sigma$}}
\newcommand{\Phim}{\hbox{\boldmath$\Phi$}}
\newcommand{\Pim}{\hbox{\boldmath$\Pi$}}
\newcommand{\Psim}{\hbox{\boldmath$\Psi$}}
\newcommand{\Thetam}{\hbox{\boldmath$\Theta$}}
\newcommand{\Omegam}{\hbox{\boldmath$\Omega$}}
\newcommand{\Xim}{\hbox{\boldmath$\Xi$}}


% Sans Serif small case

\newcommand{\asf}{{\sf a}}
\newcommand{\bsf}{{\sf b}}
\newcommand{\csf}{{\sf c}}
\newcommand{\dsf}{{\sf d}}
\newcommand{\esf}{{\sf e}}
\newcommand{\fsf}{{\sf f}}
\newcommand{\gsf}{{\sf g}}
\newcommand{\hsf}{{\sf h}}
\newcommand{\isf}{{\sf i}}
\newcommand{\jsf}{{\sf j}}
\newcommand{\ksf}{{\sf k}}
\newcommand{\lsf}{{\sf l}}
\newcommand{\msf}{{\sf m}}
\newcommand{\nsf}{{\sf n}}
\newcommand{\osf}{{\sf o}}
\newcommand{\psf}{{\sf p}}
\newcommand{\qsf}{{\sf q}}
\newcommand{\rsf}{{\sf r}}
\newcommand{\ssf}{{\sf s}}
\newcommand{\tsf}{{\sf t}}
\newcommand{\usf}{{\sf u}}
\newcommand{\wsf}{{\sf w}}
\newcommand{\vsf}{{\sf v}}
\newcommand{\xsf}{{\sf x}}
\newcommand{\ysf}{{\sf y}}
\newcommand{\zsf}{{\sf z}}


% mixed symbols
%\newcommand{\T}{{\scriptscriptstyle\mathsf{T}}}
%\newcommand{\H}{{\scriptscriptstyle\mathsf{H}}}
\newcommand{\sinc}{{\hbox{sinc}}}
\newcommand{\diag}{{\hbox{diag}}}
\renewcommand{\det}{{\hbox{det}}}
\newcommand{\trace}{{\hbox{tr}}}
\newcommand{\sign}{{\hbox{sign}}}
\renewcommand{\arg}{{\hbox{arg}}}
%\newcommand{\var}{{\hbox{var}}}
\newcommand{\cov}{{\hbox{cov}}}
\newcommand{\SINR}{{\sf SINR}}
\newcommand{\SNR}{{\sf SNR}}
\newcommand{\Ei}{{\rm E}_{\rm i}}
\renewcommand{\Re}{{\rm Re}}
\renewcommand{\Im}{{\rm Im}}
\newcommand{\eqdef}{\stackrel{\Delta}{=}}
\newcommand{\defines}{{\,\,\stackrel{\scriptscriptstyle \bigtriangleup}{=}\,\,}}
\newcommand{\<}{\left\langle}
\renewcommand{\>}{\right\rangle}
%\newcommand{\herm}{{\sf H}}
%\newcommand{\trasp}{{\sf T}}
%\newcommand{\transp}{{\sf T}}
\renewcommand{\vec}{{\rm vec}}
\newcommand{\Psf}{{\sf P}}
\newcommand{\Cov}{{\mathsf{Cov}}}
% Colors

\newcommand{\RED}{\color[rgb]{1.00,0.10,0.10}}
\newcommand{\BLUE}{\color[rgb]{0,0,0.90}}
\newcommand{\GREEN}{\color[rgb]{0,0.80,0.20}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{hyperref}
%\hypersetup{
%    bookmarks=true,         % show bookmarks bar?
%    unicode=false,          % non-Latin characters in Acrobat�s bookmarks
%    pdftoolbar=true,        % show Acrobat�s toolbar?
%    pdfmenubar=true,        % show Acrobat�s menu?
%    pdffitwindow=false,     % window fit to page when opened
%    pdfstartview={FitH},    % fits the width of the page to the window
%%    pdftitle={My title},    % title
%%    pdfauthor={Author},     % author
%%    pdfsubject={Subject},   % subject of the document
%%    pdfcreator={Creator},   % creator of the document
%%    pdfproducer={Producer}, % producer of the document
%%    pdfkeywords={keyword1} {key2} {key3}, % list of keywords
%    pdfnewwindow=true,      % links in new window
%    colorlinks=true,       % false: boxed links; true: colored links
%    linkcolor=red,          % color of internal links (change box color with linkbordercolor)
%    citecolor=green,        % color of links to bibliography
%    filecolor=magenta,      % color of file links
%    urlcolor=cyan           % color of external links
%}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Neuer Ordner/plotRNNfeatureSet.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=8.422in,
height=1.66in,
at={(0.446in,0.643in)},
scale only axis,
axis on top,
xmin=0.5,
xmax=90.5,
xlabel style={font=\color{white!15!black}},
xlabel={Time Sequence Index},
y dir=reverse,
ymin=0.5,
ymax=17.5,
ylabel style={font=\color{white!15!black}},
ylabel={Feature Index},
label style={font=\huge},
axis background/.style={fill=white}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=90.5, ymin=0.5, ymax=17.5] {plotRNNfeatureSet-1.png};
\end{axis}

\begin{axis}[%
width=11.125in,
height=2.49in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Top plot  %%%%%%%%%%%%%%%%%%

%\begin{axis}[%
%width=8.622in,
%height=1.66in,
%at={(0.446in,2.850in)},
%scale only axis,
%axis on top,
%xmin=0.5,
%xmax=90.5,
%xlabel style={font=\color{white!15!black}},
%%xlabel={Time Sequence Index},
%y dir=reverse,
%ymin=0.5,
%ymax=17.5,
%ylabel style={font=\color{white!15!black}},
%ylabel={Feature Index},
%axis background/.style={fill=white}
%]
%\addplot [forget plot] graphics [xmin=0.5, xmax=90.5, ymin=0.5, ymax=17.5] {plotRNNfeatureSet_2-1.png};
%\end{axis}
%
%\begin{axis}[%
%width=11.125in,
%height=2.49in,
%at={(0in,0in)},
%scale only axis,
%xmin=0,
%xmax=1,
%ymin=0,
%ymax=1,
%axis line style={draw=none},
%ticks=none,
%axis x line*=bottom,
%axis y line*=left
%]
%\end{axis}

\end{tikzpicture}%

==> Neuer Ordner/schematicRNN.tex <==
\begin{tikzpicture}[
             font = \sffamily,
        shorten > = 1pt,
                > = Stealth,
    node distance = 6mm and 18mm,
      start chain = going below,
 every pin/.style = {pin distance=11mm, pin edge={thin, black, ->}},
    neuron/.style = {circle, draw, fill=#1,
                     minimum size=17pt, inner sep=1pt,
                     },
     annot/.style = {text width=6em, align=center},
        BC/.style = {decorate,
                            decoration={calligraphic brace, amplitude=4pt,
                            pre =moveto, pre  length=1pt,
                            post=moveto, post length=1pt,
                            raise=6mm, mirror},
                            thick,
                            pen colour={blue}
                         }
                        ]

%%%%%%%%%%%%%%%   loop for drawing the input circles
% input variables
\foreach \i in {1,...,9}
{
 \ifnum\i=5
    \node[neuron=white,draw=none,on chain]   (in-\i)        {$\vdots$};
 \else
     \ifnum\i<10
        \node[neuron=white,on chain]             (in-\i)    {};
     \else
        \node[neuron=white,draw=none,on chain]   (in-\i)    {$\vdots$};
     \fi
 \fi
}


% Draw the rectangle
\path   let \p1 = ($(in-1.north) - (in-9.south)$),
            \n1 = {veclen(\y1,\x1)} in
        node (r) [minimum height=\n1,
                  minimum width=9mm, draw, fill=gray!10,
                  below right=0mm and 15 mm of in-1.north]
                  {\rotatebox{90}{RNN (LSTM) Layer}};
 % Draw the rectangle
\path   let \p2 = ($(in-1.north) - (in-9.south)$),
            \n2 = {veclen(\y2,\x2)} in
        node (r2) [minimum height=\n2,
                  minimum width=9mm, draw, fill=gray!10,
                  below right=0mm and 26 mm of in-1.north]
                  {\rotatebox{90}{RNN (biLSTM) Layer}};
                  
                  
                  
                  
 % Draw the rectangle
\path   let \p2 = ($(in-2.north) - (in-7.south)$),
            \n2 = {veclen(\y2,\x2)} in
        node (r3) [minimum height=\n2,
                  minimum width=9mm, draw, fill=red!10,
                  below right=18.5mm and 50 mm of in-1.north]
                  {\rotatebox{90}{Dense Layer}};
                               
 % Draw the rectangle
\path   let \p2 = ($(in-2.north) - (in-7.south)$),
            \n2 = {veclen(\y2,\x2)} in
        node (r4) [minimum height=\n2,
                  minimum width=9mm, draw, fill=green!10,
                  below right=18.5mm and 60 mm of in-1.north]
                  {\rotatebox{90}{Sigmoid Activation}};
                  
                  
                                                     
                  
 % Draw the rectangle
\path   let \p2 = ($(in-2.north) - (in-7.south)$),
            \n2 = {veclen(\y2,\x2)} in
        node (out) [minimum height=\n2,
                  minimum width=9mm, draw, fill=blue!20,
                  below right=18.5mm and 80 mm of in-1.north]
                  {\rotatebox{90}{Prediction}};
                  
                  
                  
                  
%% hidden  layer 1 neurons (circles)
%\node[neuron=gray!22,right=of in-1 -| r.east] (I-1) {};
%\node[neuron=gray!22,right=of in-3 -| r.east] (I-2) {};
%\node[neuron=gray!22,right=of in-5 -| r.east] (I-5) {};%added
%\node[neuron=gray!22,right=of in-6 -| r.east] (I-3) {};
%\node[neuron=gray!22,right=of in-7 -| r.east] (I-4) {};
%% hiden layer neurons
%\node[neuron=gray!44,right=of in-2 -| I-1.east] (H-1) {};
%\node[neuron=gray!44,right=of in-5 -| I-1.east] (H-2) {};
%\node[neuron=gray!44,right=of in-8 -| I-1.east] (H-3) {};


%% out layer neuron
%\node[neuron=gray!66,right=of r4,pin=right:Prediction] (out) {};

%% bias nodes
%\path (I-1) -| (H-1) node (B1) [pos=0.25,neuron=blue!33] {Bias};
%\path (I-1 -| H-1) -| (out) node (B2) [pos=0.25,neuron=blue!33] {Bias};


% Annotations of the layers
\node[annot,above=of in-1]  {input layer};
\node[annot,above=of r]      {Recurrent Layer};
\node[annot,above=of r3]      {Fully connected layer};
\node[annot,above=of out]    {Classification layer};

% input labels
\draw[BC] (in-1.north) --
    node[left=11mm,align=right] {Input features($\vert \vec{z}\vert$)\\ } (in-9.south) ;
%\draw[BC] (in-6.north) --
%    node[left=11mm,align=right] {$\Im (x)$} (in-9.south);

%%%%%%%%%%%%%%%%%%%%%%%%%%%%  draw the arrows
% nodes connections 
% input
\foreach \i in {1,...,4,6,7,8,9}
    {\draw[->]   (in-\i) -- (in-\i -| r.west);}
%\foreach \i in {1,3,6,7}
%    {\draw[->]   (in-\i) -- (in-\i -| r.west);}

%% input layer
%\foreach \i in {1,...,4}
%    {\draw[->]   (r3.west -| r2.east) -- (r);}

%% hidden layer
%\foreach \i in {1,...,4}
%    \foreach \j in {1,...,3}
%    \draw[->] (I-\i) edge (H-\j);

% output layer
 \foreach \i in {2}
    \draw[->] (r2) edge (r3);

% output layer
 \foreach \i in {2}
    \draw[->] (r4) edge (out);

%% bias connection.
% \foreach \i in {1,2,3}
%    \draw[->,dashed,blue!40] (B1) edge (H-\i);
%    \path[->,dashed,blue!40] (B2) edge (out);
   \end{tikzpicture}


==> Neuer Ordner/schematicRNN_sliding_window.tex <==
\begin{tikzpicture}
    [%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        box/.style={rectangle,draw=black, ultra thick, minimum size=1cm},
    ]%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    
    
\tikzset{
  boxy/.style = {rectangle,
    draw=black,
     ultra thick, 
     minimum size=1cm ,
     fill=blue!30
  }
}

\newcommand{\mywind}[1]{\node [mywind] }
    
%    
%      \newcommand*{\mywind}[1]{ [
%        box/.style={rectangle,draw=red, ultra thick, minimum size=1cm},]}
%    
%     \newcommand*{\mywinds}[1]{\fcolorbox{red}{red!20!white}{$#1$}}

\foreach \x/\y in {0/0, 1/1,2/,3/ ,4/ ,5/ ,6/ ,7/ ,8/ ,9/G-1,10/G}
        \node[box] at (\x,0){\y};
        
        \foreach \x/\y in {3/m-L,4/,5/k,6/,7/m+L}
        \node[boxy] at (\x,0){\y};
        
        \foreach \x/\y in {3/0,4/0,5/0,6/1,7/0}
        \node[box] at (\x,-3){\y};
      


\draw[decorate,decoration={brace,mirror},thick] (2.5,-.7) -- node[below]{sliding feature window (input features)} (7.5,-.7);
\draw[decorate,decoration={brace,mirror},thick] (-.5,-1.5) -- node[below]{pseudo-spectrum} (10.5,-1.50);
\draw[->,very thick] (3,1.2) --  node[above,yshift=2mm]{last element in window} (3,.7);
\draw[->,very thick] (5,1.4) --  node[above,yshift=4.5mm]{CUT} (5,.7);

\draw[<-, thick] (8,-3.0) --  node[right,xshift=3mm, yshift=0mm]{label vector} (8.5,-3.0);
%\draw[<-, thick] (8,-3) --  node[right,yshift=1mm]{input features} (8.5,-3);

\end{tikzpicture}

%\begin{tikzpicture}[font=\ttfamily,
%array/.style={matrix of nodes,nodes={draw, minimum size=7mm, fill=blue!30},column sep=-\pgflinewidth, row sep=0.5mm, nodes in empty cells,
%row 1/.style={nodes={draw=none, fill=none, minimum size=5mm}},
%row 1 column 1/.style={nodes={draw}}}]
%
%\matrix[array] (array) {
%k-L & k-L+1 & ... &  &  & k  &  & & ... & k-L+1 & k+L\\
%  &   &   &   &   &   &   &   &   &  &  \\};
%\node[draw, fill=gray, minimum size=4mm] at (array-2-9) (box) {};
%
%\begin{scope}[on background layer]
%\fill[green!10] (array-1-1.north west) rectangle (array-1-10.south east);
%\end{scope}
%
%\draw[<->]([yshift=-3mm]array-2-1.south west) -- node[below] {window Lenght is 2L+1} ([yshift=-3mm]array-2-10.south east);
%
%\draw (array-1-1.north)--++(90:3mm) node [above] (first) {First index};
%\draw (array-1-10.east)--++(0:3mm) node [right]{Indices};
%\node [align=center, anchor=south] at (array-2-9.north west|-first.south) (8) {Element\\ (at index 8)};
%\draw (8)--(box);
%%
%\end{tikzpicture}
